Phase Retrieval using Single-Instance Deep Generative Prior

Several deep learning methods for phase retrieval exist, but most of them fail on realistic data without precise support information. We propose a novel method based on single-instance deep generative prior that works well on complex-valued crystal data.

==> problem_setup.tex <==
\section{Problem Setup}

% In this paper we discuss the problem of reconstructing image $\hat{\mb X}$, from magnitude-only Fourier measurement $\mb Y$, which 

We formulated as optimization problem of the form:

\begin{align} \label{eq:passive_main}
    \min_{\mb \theta} \; \ell\paren{\mb Y, \abs{\mc F \circ G_{\mb \theta}\paren{\mb z}}^2},    \quad
\end{align}
  where the latent code $z$ is a fixed low-dimensional generic vector. In this paper, the weights $\theta$ are not \emph{pre-trained}; rather, the task is to estimate the signal $\hat{\mb X} = G_{\mb \theta}\paren{\mb z}$ and corresponding weight $\theta$, for a fixed seed $z$. Due to symmetries, the network output any symmetrical copy of ${\mb X}$ i.e. $\abs{\mc F \circ G_{\mb \theta}\paren{\mb z}}^2 \approx \mb Y $. The network $G_\theta$ takes the form of an neural network architecture similar to the one in ~\cite{heckel2018deep}. 



==> results.tex <==
\section{Experimental Results}

\begin{figure}[tp]
  \centering
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{result_images/Deep_Image.png}
    % \caption{Visualization of recovery results. First row contains complex groundtruth images, and the 2 nd and 3 rd columns are reconstructions produced by HIO and Structural Models, respectively.}
    \label{fig:result}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{result_images/two_column_comparison_natural.png}
    % \caption{}
    \label{fig:datasetbias}
  \end{minipage}
   \caption{Visualization of recovery results. (left) First row contains complex groundtruth images, (right) First row contains natural images. 2 nd and 3 rd columns are reconstructions produced by HIO and Structural Models, respectively.}
\end{figure}



In this section, we empirically show that structural models are able to accurately recover the object upto its intrinsic symmetry. We use natural images with translation (real valued) and simulated crystal dataset(complex imaged) to test our method. Simulated crystal data was generated by creating 2D convex and concave complex shapes based on random scattering points in a 110-by-110 grid within a 128-by-128 background. The phase information was determined by projecting the simulated 2D crystal defect displacement fields to the corresponding momentum transfer vectors for each reflection. We compared our method with popular iterative method HIO. Results in Figure \ref{fig:result}. Visibly, we can observe that HIO reconstruction has blurred boundary because of the translation and symmetry. We note that structural models give good recovery for both complex and real images and is able to resolve the symmetry without any difficulty.  
While this work demonstrated our approach success on simulated observations, we expect to conform its finding on experimental data in future work. 

% We acknowledge that sometimes structural models doesn not converge and in that case we rerun our model with a different z.
